Statistical Learning for OCR Text Correction

The accuracy of Optical Character Recognition (OCR) is crucial to the success of subsequent applications used in text analyzing pipeline. Recent models of OCR post-processing significantly improve the quality of OCR-generated text, but are still prone to suggest correction candidates from limited observations while insufficiently accounting for the characteristics of OCR errors. In this paper, we show how to enlarge candidate suggestion space by using external corpus and integrating OCR-specific features in a regression approach to correct OCR-generated errors. The evaluation results show that our model can correct 61.5% of the OCR-errors (considering the top 1 suggestion) and 71.5% of the OCR-errors (considering the top 3 suggestions), for cases where the theoretical correction upper-bound is 78%.

==> Makefile <==
BUILD_NAME=EACL17
BUILD_DIR=.build

# source files
TEX_FILES=$(wildcard tex/**/*.tex) main.tex preamble.tex
BIB_FILES=$(wildcard bib/**/*.bib)

# Latex compiler settings
FLAG=-quiet -f -outdir=$(BUILD_DIR) \
		 -pdf -pdflatex="pdflatex -interaction=errorstopmode" -use-make
LATEX=latexmk $(FLAG)


compile: build/EACL17/$(BUILD_NAME).pdf
.PHONY: compile

clean:
	@rm -rf $(BUILD_DIR)
.PHONY: clean

clean-all: clean
	@rm -rf build
.PHONY: clean-all

build/EACL17/$(BUILD_NAME).pdf: $(BUILD_DIR)/main.pdf build/EACL17
	@cp $< $@

$(BUILD_DIR)/main.pdf: main.tex $(TEX_FILES) $(BIB_FILES) $(BUILD_DIR)
	@echo
	@$(LATEX) $<
	@echo

$(BUILD_DIR):
	@mkdir -p $(BUILD_DIR)

build/EACL17: build
	@mkdir -p build/EACL17

build:
	@mkdir -p build

